Storyfier: Exploring Vocabulary Learning Support with Text Generation Models

Vocabulary learning support tools have widely exploited existing materials, e.g., stories or video clips, as contexts to help users memorize each target word. However, these tools could not provide a coherent context for any target words of learners' interests, and they seldom help practice word usage. In this paper, we work with teachers and students to iteratively develop Storyfier, which leverages text generation models to enable learners to read a generated story that covers any target words, conduct a story cloze test, and use these words to write a new story with adaptive AI assistance. Our within-subjects study (N=28) shows that learners generally favor the generated stories for connecting target words and writing assistance for easing their learning workload. However, in the read-cloze-write learning sessions, participants using Storyfier perform worse in recalling and using target words than learning with a baseline tool without our AI features. We discuss insights into supporting learning tasks with generative models.

==> sections/userStudy.tex <==
\section{User Study}
% Some primitive user study ideas.
\pzh{Move the current content to the Design section}
\pzh{And rewrite this section with new user study (remove most of the current results)}

\pzh{Leave the results about:}
\begin{itemize}
    \item Engagement in learning activities of three modes (significant)
    \item self-reported performance (trend), usefulness (trend) --> suggested usefulness of the three modes (not prove, but could be enough in a quick test (or other name to describe the study)?)
    \item Interview results --> Need for blending these activities
\end{itemize}

% \textbf{Study Goal.}
% understand the role of story generation models to students for English vocabulary learning in different levels of human-machine collaboration.  
To explore the user experience and effectiveness of our story-based vocabulary learning system and understand how users learn under different levels of human-machine collaboration, we conduct a within-subjects study with 12 university students. 
Specially, we evaluate three human-machine collaboration conditions in our system. In the \textit{read} case, users observe machine-generated stories to learn English vocabulary (\autoref{fig:system}A). In the \textit{cloze test} case, users complete cloze test of English words using machine-generated stories (\autoref{fig:system}B). In the \textit{turn-taking} case, users and the machine can take turns co-producing a story using all target words to learn (\autoref{fig:system}C).  
The baseline condition only provides a \textit{dictionary} function that shows the meanings, synonyms/antonyms, and usage examples for each target word (\autoref{fig:system}A1). 
Our research questions are: 

\begin{compactitem}
\item \textbf{RQ1.} How does story-based learning supported by different collaboration levels of story generation affect users' a) engagement and enjoyment in the vocabulary learning process and b) learning outcome?
\item \textbf{RQ2.} How do users perceive such story generation models for vocabulary learning?
\end{compactitem}

\subsection{Participants}
We recruit 12 junior undergraduate students (P1-12, $6$ females, $6$ males, mean age: $19.5$ (SD = $0.52$)) who majored in Artificial Intelligence in a university in mainland China via word-of-mouth. 
All of them have passed the national English exam CET-4 in China, with an average score 560.50 (SD = 37.75). 
Seven participants additionally have passed a higher level of English exam CET-6 (mean score: 510.86 (SD = 60.33) ), while two failed it and another three have not participated in it \footnote{425/710 points are considered passed for CET-4 and CET-6.}.
On average, participants self-assess their English proficiency with a score 3.50 (SD = 1.24; 1 - not proficient at all, 7 - very proficient). 


\subsection{Tasks}
Each participant is required to complete four vocabulary learning task, each under one of the four experiment conditions (i.e., \textit{dictionary, read, cloze, turn-taking}). 
In each task, participants are presented with two word groups to learn. 
Each group consists of five words from the CET-4 word corpus. 
% \zh{how to select?}. 
To decide the words for each group, we first randomly sample a story title from the ROCStory dataset and retrieve five topically related words (as described in \autoref{subsec.org_vocab}).
In the baseline \textit{dictionary} condition, participants learn the target words only using the system's dictionary function. 
In the \textit{read} condition, they can additionally read the generated story containing the target words. 
In the \textit{cloze} condition, participants can use the target words to fill in the blanks in the generated story. 
In the \textit{turn-taking} condition, participants are allowed to use the target word to co-write a story with the system by turns. 
We fix the order of presented word groups for all participants but counterbalance the order of the four experiment conditions to mitigate the ordering effects of our independent variable. 


\subsection{Measurements} 
\textbf{(RQ1a)} For each experiment condition, we measure users' perceived engagement and enjoyment in the learning process using items adapted from \cite{arguetutor,engagement}: \textit{``I was absorbed in using this version of the system to learn vocabulary in the last session''}  and \textit{``It is enjoyable to learn vocabulary with this version of the system in the last session''}. 
\textbf{(RQ1b)} We measure users' learning outcomes from two aspects: self-reported learning outcome (``I understood the meanings and usage of the two groups of target words very well in the last session'' adapted from \cite{video_vocabulary}) and retention performance 24 hours after the learning tasks. 
Specifically, we follow the work~\cite{video_vocabulary} and design a free-response vocabulary quiz consisting 40 randomly shuffled questions. 
Each question provides a word that had appeared in the learning sessions and asks participants to write down its meaning either in English or Chinese as well as a phrase or sentence that uses the word. 
If they can not quickly remember the word, they can answer ``no'' and move on to the next question. 
For each question, we additionally ask the participant to self-report whether they had known the meaning of the word before the learning session so that we could determine whether it was a new word or one they had previously. 
Two authors manually score all the responses after the study, with 1 point for a correct meaning/phrase/sentence and 0 points for the wrong one. 
\textbf{(RQ2)} We adapt the technology acceptance model \cite{AL_adaptive_learning10.1145/3313831.3376732, Technology_acceptance_model:doi:10.1111/j.1540-5915.2008.00192.x} to measure the following in each condition: \textit{usefulness} (four items, e.g., ``The use of this version of the system enables me to learn the vocabulary more efficiently''; Cronbach's $\alpha = 0.944$); \textit{easy to use} (four items, e.g., ``I would find this version of the system to be flexible to use''; $\alpha = 0.786$); and \textit{intention to use} (two items, e.g., ``If this version of the system is available there to help me learn vocabulary, I would use it''; $\alpha = 0.966$). 
We average the ratings of multiple questions as the final score for each aspect in the acceptance model. 
All statements in the questionnaires are rated on a standard 7-point Likert Scale, with 1 - strongly disagree and 7 - strongly agree. 

\subsection{Procedure}
Participants use their own computers to conduct the study following documented instructions. 
After filling out the consent form and background survey, participants read the task description about learning given vocabulary using our system. 
Then participants start experiencing the four experiment conditions one by one in a counterbalanced order. 
We allocate 3 minutes for participants to learn the two word groups in each condition 
% based on a pilot study with two users 
and tell the participants that they can finish early or take more time if needed. 
After each condition, participants rate their engagement and enjoyment in the learning process, perceived learning performance, and acceptance of the system used in this condition. 
Upon completion of four conditions, we further ask for their comments on our story-based vocabulary learning tools and their suggestions for improvement. 
One day after experiments on these four conditions, participants are also presented with a quiz asking the meaning and usage of each learned word. 
In total, each participant spent around 60 minutes in our study. 
After debriefing, each participant receives USD \$9.5 as compensation. 


\subsection{Analyses and Results}
We first check whether the order of system conditions affects our quantitative ratings via a set of mixed ANOVA tests (system order as between-subjects, system as within-subjects) on each rating. 
Neither the main effect of the system order nor its interaction effects with the tool are significant. 
Hence, in the following repeated measured ANOVA analysis, we treat the system condition (\textit{Dictionary} vs. \textit{Read} vs. \textit{Cloze} vs. \textit{Turn-taking}) as the only within-subjects variable. 
For each ANOVA, the assumption of equal variance holds according to Macuchly's test of sphericity 
\cite{ANOVA}. 

\begin{figure*}
    \includegraphics[width=\textwidth]{figures/user_study.png}
    \caption{Means and standard errors of the rated RQ1a) learning experience, RQ1b) outcome, and RQ2) technology acceptance towards different versions of vocabulary learning systems on a 7-points Likert scale ($+:.05<p<.1,*:p<.05,**:p<.01$).}
    \Description{Collaborative story writing for vocabulary learning.}
    \label{fig:user_study}
\end{figure*}

\subsection{Engagement and Enjoyment in the Learning Process (RQ1a)}
As shown in  \autoref{fig:user_study} RQ1a, participants generally feel that they are significantly more engaging in the vocabulary learning process with the \textit{Read} ($M = 5.50, SD = 1.31, p < 0.01$) and \textit{Turn-taking} ($M = 5.50, SD = 1.24, p < 0.05$) systems than that with the \textit{Dictionary} one ($M = 4.17, SD = 1.49$); $F(3, 33) = 5.14, p < 0.01, \eta^2 = 0.32$; Bonferroni post-hoc test. 
As commented by P3, \example{The Dictionary system gives too many details for each word, and this will increase the burden to learn all target words.
% gives the positive and negative synonyms of words, and this will increase the burden of learners. 
Also, it is difficult for me to concentrate for a long time. But I can be immersed in the story context through the Reading system.} P7 and P11 said, \example{The Turn-taking system increases interactivity, making me engage myself in learning with lots of fun.}
Furthermore, there is a significant difference in perceived enjoyment in the learning process with four systems; $F(3, 33) = 2.88, p < 0.05, \eta^2 = 0.21$. 
The Bonferroni post-hoc test shows that with a marginally significant difference, participants feel more enjoyable learning with the \textit{Read} ($M = 5.25, SD = 1.48, p = 0.052$) system than that with the \textit{Dictionary} one ($M = 4.00, SD = 1.41$). 
\example{The Dictionary system is too traditional and boring.} (P3).


\subsection{Learning Outcome (RQ1b)} 
\textbf{Self-reported learning outcome.} 
As shown in \autoref{fig:user_study} RQ1b, there is a marginally significant difference in self-reported learning performance with four systems; $F(3, 33) = 2.80, p = 0.055, \eta^2 = 0.20$. 
The Bonferroni post-hoc test reveals that on average, participants feel that they perform better using the \textit{Read} ($M = 5.17, SD = 1.19, p = 0.084$) system than that using the \textit{Dictionary} one ($M = 3.92, SD = 1.51$). 
\example {The Reading system displays words through stories written by the system. This helps me better understand the usage of words. (P3 and P12)}. 

\textbf{Retention performance.} 
Since the vocabulary quiz answers were done in free-response format, a third-party Ph.D. student who is fluent in English and Chinese was asked to mark the learners' quiz answers as being either correct or incorrect. 
The grader was blind as to which condition or which learner the answer was coming from. 
We measure the number of correctly defined words, the number of correctly used words, and the number of words that participants had marked as previously known. 
% As shown in Fig. xxx \zh{To do by Zhenhui}
The results show that the numbers of correctly defined English words are similar in all four conditions; means of \textit{Dictionary} vs. \textit{Read} vs. \textit{Cloze} vs. \textit{Turn-taking}: $8.83 (SD=0.72)$ out of $10$ total, $9.00 (0.85), 9.08 (0.79), 9.17 (0.83)$; $F(3,33)=0.55, p = 0.65, \eta^2=0.05$. 
Excluding the words that participants had marked as previously known, the numbers of newly learned and correctly defined words are also similar in four cases: $1.08 (1.16), 1.08 (1.24), 1.08 (1.62), 0.92 (1.24)$; $F(3,33)=0.06, p = 0.98, \eta^2=0.01$. 
These results suggest that our participants have learned the meanings of vocabulary well before and during the experiments, regardless of the system conditions. 
However, we observe a marginally significant difference across four systems in terms of the numbers of correctly used (in users' written phrases or sentences) words; $F(3,33)=2.28, p = 0.097, \eta^2=0.172$. 
The Bonferroni post-hoc test further indicates that \textbf{with \textit{Turn-taking} ($M = 8.92, SD = 1.08$) system, participants could better master the usage of words, }in comparison to the \textit{Dictionary} ($M = 8.00, SD = 1.48, p<0.05$), \textit{Read} ($M = 8.08, SD = 1.68,p<0.05$), and \textit{Cloze} systems ($M = 8.25, SD = 1.22,p<0.05$). 

\subsection{Acceptance Towards the Story-Based Vocabulary Learning System (RQ2)}
\textbf{Usefulness.} As shown in \autoref{fig:user_study} RQ2, participants feel significantly different regarding the usefulness of our four systems; $F(3, 33) = 3.83, p < 0.05, \eta^2 = 0.26$. 
Specifically, they feel that the \textit{Read} ($M = 4.94, SD = 1.15, p < 0.05$) system is significantly more useful that the \textit{Dictionary} one ($M = 3.56, SD = 1.45$); Bonferroni post-hoc test. 
P3, P4, P7, and P12 reflected that the vocabulary learning process with the Dictionary one is tedious. They can easily give up in this way. Especially P4 pointed, \example{It is better to read books directly instead of reciting words through the Dictionary system.}

\textbf{Easy to use.} 
As for the second aspect of technology acceptance model, participants feel that the \textit{Read} ($M = 4.83, SD = 1.12, p < 0.01$) system is significantly easier to use than the \textit{Turn-taking} one ($M = 3.15, SD = 0.85$); $F(3, 33) = 9.54, p < 0.001, \eta^2 = 0.46$; Bonferroni post-hoc test. 
Besides, the \textit{Cloze} ($M = 4.27, SD = 1.13, p < 0.05$) system is deemed significantly easier to use than the \textit{Turn-taking} one, and there is a marginal significantly higher rating result of \textit{Read} system than the \textit{Dictionary} one ($M = 4.19, SD = 1.28, p = 0.083$). 
P8 and P11 indicated that sometimes they cannot immediately think of how to use words to write a story sentence, which wastes some time. But in the \textit{cloze} system, words only need to be filled in. This reduces the workload and allows them to better grasp the words and their usage in a shorter time.

\textbf{Intention to use.} 
Lastly, participants have significantly higher intentions to use the \textit{Read} ($M = 4.71, SD = 0.33$) system for their vocabulary learning in the future, compared to the \textit{Dictionary} ($M = 2.96, SD = 1.63, p < 0.01$) and \textit{Turn-taking} systems ($M = 3.13, SD = 1.40, p < 0.05$); $F(3, 33) = 5.80, p < 0.01, \eta^2 = 0.35$; Bonferroni post-hoc test. 
P2, P5, P8, P11, and P12 commented that it is still demanding for users to create logically coherent stories even with the help of the machine in the \textit{turn-taking} condition.
% requires users to create a logically coherent story. It is very demanding for learners. 
And some of them feel tired in this process. P4 suggested \example{The \textit{turn-taking} system is more like a review and practice system. Learners can consolidate and master the learned words through it.}


% \textbf{Research Questions.}
% \begin{compactitem}
% \item \textbf{RQ1.} How do different collaboration levels of story generation affect students’ a) perception and behaviors in the vocabulary learning process and b) learning outcome?
% \item \textbf{RQ2.} How do students use and perceive such story generation models for vocabulary learning?
% \end{compactitem}


% \subsection{Alternative}
% An alternative design of evaluation. Ablation study of using the system or NOT in the scenario of using story to learn a set of vocabulary.

% \begin{compactitem}
% \item \textbf{Control group.}
% Users are provided with only dictionary support for looking up vocabulary. They are required to learn a set of vocabulary of (\xb{with possible writing feedback?}).

% \item \textbf{Experimental group.} 
% Besides the functions provided by a baseline system in control group, 
% users can use machine-generated stories for vocabulary learning in different levels of human-machine collaborations, from passive observation, cloze test, to interactively co-producing stories with machine.

% \end{compactitem}
